Lattice QCD Thermodynamics with Physical Quark Masses

Over the past few years new physics methods and algorithms as well as the latest supercomputers have enabled the study of the QCD thermodynamic phase transition using lattice gauge theory numerical simulations with unprecedented control over systematic errors. This is largely a consequence of the ability to perform continuum extrapolations with physical quark masses. Here we review recent progress in lattice QCD thermodynamics, focussing mainly on results that benefit from the use of physical quark masses: the crossover temperature, the equation of state, and fluctuations of the quark number susceptibilities. In addition, we place a special emphasis on calculations that are directly relevant to the study of relativistic heavy ion collisions at RHIC and the LHC.

==> lqcd_thermo_3_methods.tex <==
\section{Lattice QCD Observables and Analytical Methods [4 pages]}
\label{sec:methods}
\subsection{QCD Phase Diagram and Transition Order}
\subsection{Chiral symmetry: condensate and susceptibility}
\subsection{Confinement: Polyakov loop, quark number susceptibility}
\subsection{$U(1)_A$ symmetry}
\subsection{Equation of State}
\subsection{Color screening}

